Exact Philosophy of Space-Time

Starting from Bunge's (1977) scientific ontology, we expose a materialistic relational theory of space-time, that carries out the program initiated by Leibniz, and provides a protophysical basis consistent with any rigorous formulation of General Relativity. Space-time is constructed from general concepts which are common to any consistent scientific theory and they are interpreted as emergent properties of the greatest assembly of things, namely, the world.

==> PaxHeader/EPhSpT.tex <==
20 ctime=1317063134
20 atime=1317063135
19 SCHILY.dev=2053
22 SCHILY.ino=3055845
18 SCHILY.nlink=1
88 LIBARCHIVE.xattr.security.selinux=dW5jb25maW5lZF91Om9iamVjdF9yOnVzZXJfaG9tZV90OnMwAA

